Safe Neighborhood Computation for Hybrid System Verification

For the design and implementation of engineering systems, performing model-based analysis can disclose potential safety issues at an early stage. The analysis of hybrid system models is in general difficult due to the intrinsic complexity of hybrid dynamics. In this paper, a simulation-based approach to formal verification of hybrid systems is presented.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{M. Bujorianu (Ed.) and R. Wisniewski (Ed.): 4th Workshop on\\ Hybrid Autonomous Systems 2014 (HAS 2014).\\
EPTCS 174, 2015, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.174.1}{10.4204/EPTCS.174.1}}
\pdfoutput=1

